Scaling Robot Policy Learning via Zero-Shot Labeling with Foundation Models

A central challenge towards developing robots that can relate human language to their perception and actions is the scarcity of natural language annotations in diverse robot datasets. Moreover, robot policies that follow natural language instructions are typically trained on either templated language or expensive human-labeled instructions, hindering their scalability. To this end, we introduce NILS: Natural language Instruction Labeling for Scalability. NILS automatically labels uncurated, long-horizon robot data at scale in a zero-shot manner without any human intervention. NILS combines pretrained vision-language foundation models in order to detect objects in a scene, detect object-centric changes, segment tasks from large datasets of unlabelled interaction data and ultimately label behavior datasets. Evaluations on BridgeV2, Fractal, and a kitchen play dataset show that NILS can autonomously annotate diverse robot demonstrations of unlabeled and unstructured datasets while alleviating several shortcomings of crowdsourced human annotations, such as low data quality and diversity. We use NILS to label over 115k trajectories obtained from over 430 hours of robot data. We open-source our auto-labeling code and generated annotations on our website: http://robottasklabeling.github.io.

==> Play_Labeling_Cam_Ready_arXiv/chapters/acknowledgements.tex <==
\acknowledgments{The work presented here was funded by the German Research Foundation (DFG) – 448648559. 
The authors acknowledge support by the state of Baden-Württemberg through HoreKa supercomputer funded by the Ministry of Science, Research and the
Arts Baden-Württemberg and by the German Federal Ministry of Education and Research.}


==> Play_Labeling_Cam_Ready_arXiv/chapters/bridge_vis.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_1/0.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_1/7.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_1/15.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_1/24.jpg_annotated.jpg}
    \end{subfigure}
    \\
    \caption*{ \textbf{Instructions generated by \gls{nils}:}
    "Move the pepper from inside the strainer to in front of the strainer", "Take the pepper out of the strainer and place it forward", "Relocate the pepper to a position in front of the strainer"\\
\textbf{Instructions generated by Gemini Vision Pro}: "Move the yellow bell pepper to the left", "Place the yellow bell pepper in the pot", "Move the pot to the right."
}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_2/0.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_2/6.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_2/12.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_2/19.jpg_annotated.jpg}
    \end{subfigure}
    \\
    \caption*{\textbf{Instructions generated by \gls{nils}:} "Place the saucepan on top of the dishrag", "Move the saucepan to the right of the soap", "Position the saucepan behind the ladle."\\
\textbf{Instructions generated by Gemini Vision Pro}: "Move the cheese to the right", "Move the bowl to the right", "Move the spoon to the right", "Move the dishrag to the right."
}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_3/0.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_3/6.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_3/13.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_3/20.jpg_annotated.jpg}
    \end{subfigure}
    \caption*{\textbf{Instructions generated by \gls{nils}:} 
    "Move the sushi from on top of the dishrag to a new location away from the saucepan", "Relocate the sushi to clear the area on top of the dishrag", "Shift the sushi to organize the workspace, ensuring it is no longer next to the saucepan."\\
\textbf{Instructions generated by Gemini Vision Pro}:
"The robot moved the green spatula from the left of the cutting board to the right of the cutting board",
"The robot moved the yellow cloth from the right of the cutting board to the left of the cutting board",
}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_4/0.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_4/3.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_4/5.jpg_annotated.jpg}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width = \textwidth]{images/evaluation/bridge_v2_qualitative/example_4/8.jpg_annotated.jpg}
    \end{subfigure}
    \caption*{\textbf{Instructions generated by \gls{nils}:} "Put the reamer (juicer) inside the plate", "Move the reamer (juicer) from next to the plate to inside it", "Place the reamer into the plate for storage or preparation"\\
\textbf{Instructions generated by Gemini Vision Pro}: "The robot picked up a carrot that was resting on a green plate and placed it in the sink.",
"The robot moved a carrot from a green plate to the sink."}
    \caption{Comparison of generated labels for samples form the bridge V2 dataset. We show the labels generated by \gls{nils} and Gemini Pro for several tasks. }
    \label{fig:combined-bridge-labels-comparison}
\end{figure}


==> Play_Labeling_Cam_Ready_arXiv/chapters/calvin_keystate_vis.tex <==
\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\linewidth]{images/evaluation/calvin_keystate_examples/0.jpeg}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\linewidth]{images/evaluation/calvin_keystate_examples/1.jpeg}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\linewidth]{images/evaluation/calvin_keystate_examples/2.jpeg}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\linewidth]{images/evaluation/calvin_keystate_examples/3.jpeg}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\linewidth]{images/evaluation/calvin_keystate_examples/4.jpeg}
       
    \end{subfigure}
    
    \vspace{1em}
   
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\linewidth]{images/evaluation/calvin_keystate_examples/0_2.jpeg}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\linewidth]{images/evaluation/calvin_keystate_examples/1_2.jpeg}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\linewidth]{images/evaluation/calvin_keystate_examples/2_2.jpeg}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\linewidth]{images/evaluation/calvin_keystate_examples/3_2.jpeg}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\linewidth]{images/evaluation/calvin_keystate_examples/4_2.jpeg}
       
    \end{subfigure}
    
    \caption{Visualization of keystates extracted by \gls{nils} for the CALVIN environment. 
    Keystates are extracted only via RGB Images, without incorporating gripper-close signals.
    In the second sequence, some intermediate keystates are not detected. Nevertheless, the predicted keystates are precise.}
\end{figure}



==> Play_Labeling_Cam_Ready_arXiv/chapters/conclusion.tex <==
\section{Discussion}

\textbf{Limitations.} 
Despite \gls{nils}' ability to generate high-quality labels, some limitations remain:
Using multiple models for generating scene representations results in a significant computational cost, requiring 7 minutes to label one  8-minute long-horizon trajectory consisting of 50 tasks on a 3090 RTX GPU.
Correlated heuristics can sometimes lead to high-confidence keystates triggered by noise, resulting in incorrect labels.
Grounding accuracy is limited by the performance of pretrained models.
\gls{nils} has high objectness assumptions for labeling, making it challenging to label tasks with granular objects and distinguish between visually similar objects due to the limitations of object detectors.

\textbf{Conclusion.}
This work introduces \gls{nils}, the first framework to autonomously label long-horizon robot datasets without human intervention or any model training. \gls{nils} offers a \textbf{cost-effective} alternative to annotate robot demonstrations compared to crowd-sourcing.
Our experiments and extensive ablations showcase \gls{nils}' capability to generate labels of \textbf{high quality} and \textbf{diversity}, enabling efficient and scalable language-conditioned robot learning.






==> Play_Labeling_Cam_Ready_arXiv/chapters/evaluation.tex <==

\section{Evaluation}
In this section, we address the central question: \textit{Can \gls{nils} generate semantically meaningful, detailed, and adjustable-granularity language annotations for existing robot interaction datasets?}
To answer this question, we assess \gls{nils}' accuracy in labeling long-horizon robot data, keystate quality, and grounding performance against state-of-the-art VLMs and study the generated task labels with respect to various properties.
\gls{nils} was evaluated on three datasets: (1) the BridgeV2 \cite{walke2024bridgedata} containing ~1200 long-horizon trajectories with 28K short horizon pick and place and state-manipulation tasks with diverse scenes, tasks, and objects; (2) Fractal \cite{brohan2022rt}, a dataset consisting of 87K short horizon demonstrations; (3) a self-collected one-hour long-horizon, uncurated play dataset in a robot play kitchen, containing 439 short-horizon demonstrations of $12$ tasks. The dataset consists of multiple long-horizon demonstration videos where the robot solves at least 10 manipulation tasks in a row.



\subsection{Keystate Evaluation}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim=1.0cm 1.0cm 1.0cm 1.0cm]{images/evaluation/keystate_plots/Kitchen_Play-1.pdf}
        \label{fig:keystates_kitchen}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim=1.0cm 1.0cm 1.0cm 1.0cm]{images/evaluation/keystate_plots/BridgeV2-2.pdf}
        \label{fig:keystates_bridge}
    \end{subfigure}
    \vspace{-0.3cm}
    \caption{Keystate accuracy for different frame distance tolerances on: Kitchen Play and BridgeV2.  
    We report the precision and recall of our method at two different keystate thresholds. 
    \gls{nils} generates relevant keystates on both datasets and surpasses both baselines.}
    \label{fig:keystates_combined}
\end{figure}
 
We quantitatively evaluate the keystates produced by \gls{nils} on both datasets using precision, recall, and mean-average precision (mAP) metrics. A predicted keystate is considered correct if its distance to a ground truth keystate is smaller than a threshold based on the average short-horizon task length. \autoref{fig:keystates_combined} shows that our framework outperforms UVD \cite{zhang2023universal} and Uniform Sampling on the Kitchen Play and BridgeV2 at a keystate threshold of $\theta_o = 0.25$. 
Incorporating gripper-close signals further improves performance, highlighting the importance of including proprioceptive information for detecting keystates, if available.
These experiments show \gls{nils} can extract valuable keystates in challenging environments.


\subsection{Grounding Evaluation}

We evaluate the grounding capabilities of \gls{nils} on a mixture of the BridgeV2 dataset and our Kitchen Play dataset.
Specifically, we select $14$ different long-horizon play demonstrations from various settings, each containing $20$ tasks.
Of these, $12$ trajectories are sampled from BridgeV2. 
We chose trajectories from diverse settings, including kitchens, tables, and washing machines, with a wide variety of objects to ensure maximal task diversity.
Further, we added two long-horizon demonstrations from our Kitchen Play Dataset with $24$ tasks each.
Given the ambiguity of language annotations, we employ human evaluators to assess whether a language label proposed by a method is correct given the segmented task video.

\begin{wraptable}{r}{0.4\textwidth}
\centering
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule
Method & GT Keystates & Accuracy \\
\midrule
XLIP & \checkmark & 0.05 \\
VideoLLava & \checkmark & 0.03 \\
Gemini 1.5 & \checkmark & 0.16\\
GPT-4o & \checkmark & 0.51 \\
NILS  & x & \textit{0.66} \\
NILS  & \checkmark & \textbf{0.84} \\
\midrule
NILS - TA & x  & 0.46 \\
NILS - MFOR & x& 0.38 \\
NILS - DI & x & 0.47\\
\bottomrule
\end{tabular}%
    }
\caption{Grounding accuracy of \gls{nils} on our mixed dataset compared against baselines and ablations. \gls{nils} outperforms all baselines by a wide margin. TA: Temporal Aggregation, MFOR: Multi Frame Object Retrieval, DI: Depth Information. GT: Ground Truth Key States.}
\label{tab:grounding_main}
\end{wraptable}
\textbf{Baselines.} We compare against four baselines. 
First, \textbf{Gemini Vision Pro} and \textbf{GPT-4o}, two large vision language models with video-understanding capabilities \cite{geminiteam2023gemini}. 
The prompt used to query these models is provided in \autoref{sec:app_prompts}.
We further test against \textbf{XCLIP}, a video-language retrieval model \cite{ma2022xclip} and \textbf{VideoLLava}, a recent open-source VLM \cite{lin2023videollava}.
Since VLMs can not segment long-horizon demonstrations out-of-the-box, we provide the baselines with ground-truth keystates to assess their grounding capabilities.


\textbf{Results.} \gls{nils} outperforms all baselines in both settings (\autoref{tab:grounding_main}).
The baselines struggle to ground the robot's actions due to the domain shift between the challenging static camera robot environment and pretraining data, consistent with previous findings \cite{sermanet_robovqa_2023,wang2024mementos,guan2024task,karamcheti_prismatic_2024}.
GPT-4o is the best-performing baseline, highlighting the performance difference compared to open-source VLMs. We found that the VLMs often correctly capture the interacted object but fail to perform correct temporal reasoning.
Additionally, we observed that VLMs tend to successfully predict high-level state changes, such as opening or closing objects, but struggle with more nuanced interactions.



\subsection{Labeling Results for BridgeV2 Dataset}
To assess the scalability of \gls{nils}, we applied it to a larger, more diverse dataset. 
Therefore, we label a subset of BridgeV2 that consists of $31K$ trajectories in diverse environments. 
The cost for \gls{nils} to label this subset was approximately $200$ USD, compared to about $5000$ USD for crowd-sourced labels\footnote{Based on the reported labeling cost of approximately $10,000$ USD for the full dataset.}.
This demonstrates the \textbf{low-cost} of \gls{nils}. 
To analyze the diversity of generated labels, we visualized the top $60$ labels, sorted by frequency, in \autoref{sec:diversity-comparison}.
This visualization confirms the \textbf{diversity} of labels generated by \gls{nils} compared to crowd-sourced annotations.
Additionally, our ablation experiments in \autoref{sec:granulaity ablations} showcase \gls{nils}'s ability to generate task labels at various \textbf{granularities}, further highlighting its flexibility.


\subsection{Language-conditioned Policy Training}


\begin{table}[h]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{c|cc|c|cc|cc|cc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Simulation}} & \multicolumn{6}{c}{\textbf{Bridge - Real Robot}} \\
\cline{2-10}
 & \multicolumn{2}{c|}{\textbf{Bridge}} & \textbf{Fractal} & \multicolumn{2}{c|}{\textbf{Spoon on Towel}} & \multicolumn{2}{c|}{\textbf{Sushi in Bowl}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cline{2-10}
 & \textbf{Success} & \textbf{CG} & \textbf{Success} & \textbf{Success} & \textbf{CG} & \textbf{Success} & \textbf{CG} & \textbf{Success} & \textbf{CG} \\
\hline
Gemini & 0\% & 11\% & - & - & - & - & - & - & - \\
GT & \textbf{4.2\%} & \textbf{41.7\%} & 1.9\% & 60\% & 93\% & 60\% & 73\% & 60\% & 83\% \\
NILS & 2.8\% & 29.6\% & \textbf{3.1\%} & \textbf{66\%} & \textbf{100\%} & 60\% & \textbf{80\%} & \textbf{63\%} & \textbf{90\%} \\
\hline
\end{tabular}%
}
\caption{Success rates for simulated (left) and real environments (right) across different tasks. We evaluate all methods on grounding ability (CG) and task success rate. Results are averaged over 15 rollouts for each task in the real robot environments.}
\label{tab:combined_methods_tasks}
\end{table}


To study the generalization of \gls{nils} for large-scale, diverse datasets, we train a language-conditioned policy with labels from \gls{nils} on the BridgeV2 \cite{walke2024bridgedata}, and Fractal \cite{brohan2022rt} datasets. 
We use Octo \cite{octo_2023}, a recent open-source diffusion policy and train it using $3$ different label sets: crowd-sourced labels (GT), \gls{nils} labels, and Gemini labels. 
We train Octo \cite{octo_2023} on different data mixtures to evaluate the capabilities of our labeling framework for downstream policy learning. In particular, we train Octo on the subset of BridgeV2 labeled by NILS and Fractal fully labeled by \gls{nils}. We always train the baseline policies with the same datasets, but switch out the language labels with their respective counterparts. Due to labeling costs and Gemini's low performance, we omit labeling Fractal with Gemini. 
Further evaluation details are provided in \autoref{sec:app_eval}.



\textbf{Results.}
The results of this experiment are summarized in \autoref{tab:combined_methods_tasks}.
In the simulated environment, our method outperforms the policy trained on labels generated by Gemini by 19\% in terms of correct grounding and 2.8\% in terms of success rate while being slightly behind the crowd-sourced annotated dataset for BridgeV2. On Fractal, the policy trained with \gls{nils} labels outperforms the policy trained on ground-truth labels by 1.1\%.
For the real robot tasks, the policy trained with labels from \gls{nils} achieves the highest average performance with a 63\% success rate.
These results align with our findings in the previous section on label accuracy.
Our experiments demonstrate that current VLMs alone are insufficient to produce high-quality labels for effective policy training.
Furthermore, these results highlight that \gls{nils} generates labels of \textbf{high quality} even for diverse, large-scale datasets, making it a promising approach for scalable robot learning.

\subsection{Ablation Studies}


\textbf{What are the most crucial components of \gls{nils}?}

\begin{wraptable}{r}{0.35\textwidth}
    \centering
    \resizebox{0.35\textwidth}{!}{%
    \begin{tabular}{@{}lc@{}}
        \toprule
        Method & Captured Objects\\
        \midrule
        Ours (Gemini) & \textbf{0.94} \\
        Ours (Gemini) + SOM & 0.74 \\
        Ours (GPT4V) & 0.67 \\
        Ours (Prismatic \cite{karamcheti_prismatic_2024}) & 0.48 \\
        \midrule
        Single Frame (Gemini) & 0.70 \\
        OWLv2 + SigLIP & 0.63 \\
        \bottomrule
    \end{tabular}%
    }
    \caption{Ablation of the effectiveness of our initial object retrieval measured in recall.
    }
    \label{tab:stage1_ablations}
\end{wraptable}
We conduct ablation studies to investigate the importance of various design decisions in \gls{nils}.
Results are summarized in the lower half of \autoref{tab:grounding_main}.
Without multi-frame object retrieval in Stage 1, \gls{nils} achieves only half the grounding accuracy, highlighting the importance of accurate and complete initial object labels.
Our experiments also indicate that the depth information provided by the zero-shot depth prediction model (DI) in Stage 2 is crucial for accurate spatial reasoning, enabling more precise task labeling.
Given the current limitations of foundation models, we found that temporal aggregation (TA) is essential for obtaining reliable and consistent bounding boxes and segmentation masks across frames.
Thorough ablations for every design decision in all Stages of \gls{nils} are provided in \autoref{sec:ablations-appendix}, confirming the importance of each Stage for achieving accurate labels.

\textbf{How to retrieve all relevant objects in the scene?} To reason about robot-object interactions, it is crucial to detect all relevant objects in the scene. We investigated various VLMs and combinations for object retrieval in Stage 1. 
We compare \gls{nils} design using Gemini with \textit{co-occurence} and \textit{detection alignment} against several variants using other VLMs like GPT-4V and open-source baseline Prismatic \cite{karamcheti_prismatic_2024}. 
Additionally, we tested a combination of popular open-source open-vocabulary models: SigLip \cite{zhai2023sigmoid} + OwlV2 \cite{minderer_scaling_2023}.
To assess the effectiveness of all approaches, we create a diverse dataset consisting of the BridgeV2 and our Kitchen Play dataset. 
In total, the ablation dataset comprises $185$ objects in various scenes. 
The results for this experiment are summarized in \autoref{tab:stage1_ablations}. 
Naively querying a VLM for a single frame does not reliably capture all objects, especially in cluttered scenes.
NILS without co-occurrence and detection alignment, denoted as ``Single Frame'', only captures $70\%$ of the objects present in the scenes, emphasizing the importance of filtering and improving initial object detections. 
While OWLv2+SigLIP presents a viable alternative, it requires prior knowledge about objects that might appear in the scene.
We also ablate Set of Mark Prompts (SOM) \cite{yang_set--mark_2023}, with our method, but found that this harms performance.












==> Play_Labeling_Cam_Ready_arXiv/chapters/introduction_rudi.tex <==

 
\section{Introduction}



\begin{figure*}[h]
     \centering
     \includegraphics[width=\linewidth]{images/introduction/Lupus_Figure_1v3.pdf}
     \caption{\textbf{A framework to label long-horizon robot demonstrations without human annotations or model training from RGB videos.} 
     NILS leverages an ensemble of frozen pretrained models to segment and annotate uncurated, long-horizon demonstrations. 
     The resulting labeled and segmented dataset can be used to train language-conditioned policies without human annotation.}
     \label{fig:enter-label}
 \end{figure*}

\looseness-1
Natural language is an intuitive and flexible interface for humans to communicate tasks to robots. 
Recent works have shown promising results in training language-conditioned policies using large datasets of robot trajectories paired with language annotations. 
However, the performance and diversity of behaviors learned by language-conditioned policies hinge critically on the quality and quantity of the language annotations. 
Unfortunately, most available robot interaction datasets do not contain any associated language annotations due to the costly nature of generating these. 
Concretely, most labeled datasets often rely on post-hoc crowd-sourced language labeling to generate labeled data~\citep{walke2024bridgedata, mees2022calvin, khazatsky2024droid, lynch2023interactive}, which has several limitations: high cost in terms of time and money, variable quality of generated labels, reduced diversity when using templated instructions, and inconsistent granularity of annotations.
The \textbf{quality} of the generated labels can vary significantly, from detailed descriptions to url links\footnote{BridgeV2 dataset contains this annotation: "\url{https://www.youtube.com/watch?v=JWA5hJl4Dv0}"}. 
This issue can be addressed through templated language instructions \cite{brohan2022rt}, which in turn reduces the the \textbf{diversity} of the annotations, i.e., the same phrasing and instruction is used for every instance of the same skill, object or spatial relation.
The least apparent downside of manually labeled behavior is the \textbf{granularity} of the annotations. 
The behavior description along the temporal axis can vary significantly from individual actions to whole multi-step tasks, e.g. \texttt{move left} and \texttt{clean the kitchen}, hence directly affecting the learned skills.
This raises the question, can we find a more scalable and cost-effective way to generate semantically meaningful, detailed, and adjustable-granularity language annotations for existing robot interaction datasets?

One option is leveraging the semantic knowledge of Vision-Language Models (VLMs) pretrained on Internet-scale data \cite{yu_scaling_2023, zhai2023sigmoid, luddecke_image_2022}.
These foundation models have found applications in different robotic contexts ~\cite{shafiullah_clip-fields_2022, chen_open-vocabulary_2022, reuss2023multimodal, liu2024ok, huang23vlmaps, ahn2022can, huang23avlmaps, chen2024vision, sermanet_robovqa_2023, Zawalski24-ecot,hirose24lelan}.
However, none of the existing models can accurately label robot demonstrations. 
Current VLMs struggle segmenting long-horizon demonstrations and tempo-spatial reasoning, especially in challenging robotic domains \cite{sermanet_robovqa_2023,chen_spatialvlm_2024}.


\looseness-1
To address these limitations, we introduce \gls{nils}, the first comprehensive system for zero-shot labeling of long-horizon robot videos without human intervention or additional model training.
\gls{nils} employs an ensemble of pretrained foundation models to identify relevant objects and generate potential task labels. \gls{nils} first identifies object-centric keystates, segmenting long videos with multiple tasks into smaller single-action windows. 
Next, a Large Language Model (LLM) generates free-form language annotations based on structured observation descriptions. These descriptions are based on templated language generated from scene changes tracked by the pretrained foundation models.
As a result, \gls{nils} converts videos of long-horizon robot interaction data into segmented and annotated datasets, which can be utilized for training language-conditioned policies without manual labeling.
Furthermore,  \gls{nils} addresses all of the above shortcomings, i.e., \textbf{cost}, \textbf{quality}, \textbf{diversity}, and \textbf{granularity}.


We demonstrate through extensive experiments, 
that \gls{nils} efficiently annotates unlabeled robot interaction data with appropriate task descriptions, surpassing state-of-the-art closed-source VLMs like Gemini-Pro. 
\gls{nils} reliably finds important keystates in long-horizon demonstrations better than prior zero-shot methods~\cite{zhang2023universal}. We demonstrate the scalability of \gls{nils} by labeling over 115k trajectories from different datasets, totaling 430 hours of robot data.
Finally, we demonstrate the effectiveness of our approach by training language-conditioned manipulation policies on the automatically labeled data on a real robot. 



==> Play_Labeling_Cam_Ready_arXiv/chapters/policy_table.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Task}   & \multicolumn{2}{c}{\textbf{Human}} & \multicolumn{2}{c}{\textbf{NILS}} & \multicolumn{2}{c}{\textbf{NILS Noisy}} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                & Grounding & Success & Grounding & Success & Grounding & Success \\ 
\midrule
banana in sink  & 1.0       & 0.67    & 1.0       & 1.0     & 1.0       & 1.0    \\
pot right       & 1.0       & 1.0     & 1.0       & 1.0     & 1.0       & 0.67   \\
pot left        & 1.0       & 0.67    & 1.0       & 0.67    & 1.0       & 0.33   \\ 
open microwave  & 1.0       & 1.0     & 0.67      & 0.67    & 0.0       & 0.0    \\
open oven       & 1.0       & 0.0     & 1.0       & 0.0     & 1.0       & 0.0    \\
open fridge     & 1.0       & 0.0     & 1.0       & 0.0     & 1.0       & 0.33   \\
close microwave & 1.0       & 1.0     & 1.0       & 1.0     & 0.67      & 0.67   \\
close oven      & 1.0       & 1.0     & 1.0       & 0.67    & 0.0       & 0.0    \\
close fridge    & 0.67      & 0.33    & 1.0       & 0.67    & 0.33      & 0.33   \\
banana on stove & 1.0       & 0.33    & 0.33      & 0.0     & 0.0       & 0.0    \\
banana oven     & 0.0       & 0.0     & 0.0       & 0.0     & 0.0       & 0.0    \\
pot in sink     & 1.0       & 0.67    & 1.0       & 0.0     & 1.0       & 0.0    \\        
\bottomrule
\end{tabular}
\caption{Relative performance for task groundings and successful task completions. 
We report the average performance of all tested tasks, where the first number depicts the relative number of correctly grounded tasks, and the second the relative number of successful completions.}
\label{tab:grounding_policy}
\end{table}





==> Play_Labeling_Cam_Ready_arXiv/chapters/related_work.tex <==


\section{Related Work}

\textbf{Key State Identification.}
Identifying important keystates from long-horizon tasks is crucial for efficiently learning goal-conditioned policies. 
Some approaches use proprioceptive observations \cite{borjadiaz2022affordance, mees_grounding_2023,james2022qattention,shridhar2022perceiveractor} or waypoint reconstruction loss \cite{borjadiaz2022affordance}.
UVD utilizes the latent space of pretrained image embedding models such as CLIP \cite{zhang2023universal} to detect keystates.
Similar to \gls{nils}, it also does not require any robot signals.
However, \gls{nils} additionally incorporates more specific information, which significantly improves keystate quality.
REFLECT \cite{liu_reflect_2023} constructs a scene graph with object relations and states, labeling frames as keyframes when the graph changes. 
However, this method relies on ground truth state information and object positions, which are usually only available in simulated environments. 
\gls{nils} detects keystates in real-world environments from robot videos only. 

\textbf{Action Recognition.}
Video action recognition involves retrieving actions performed over multiple frames, either through dense video action recognition (extracting multiple actions and their time frames) or video action classification (assuming a single action per video). 
Generalist VLMs can solve these tasks in a zero-shot, open-vocabulary manner \cite{yang2023vid2seq,yan_videococa_2023,wang2022language,fang_clip2video_2021,ko_large_2023}.
RoboVQA \cite{sermanet_robovqa_2023} finetunes a video VLM on a labeled robot demonstration VQA dataset to answer questions about robot actions in robotics.
REFLECT \cite{liu_reflect_2023} extracts scene graphs that could be used for action retrieval but assume a known robot plan to analyze robotic failure cases.
Several works fine-tune CLIP \cite{xiao_robotic_2023, myers_goal_2023, ge_policy_2023,  ma_liv_2023} using a small subset of domain-specific data.
These CLIP models then retrieve actions for a larger, unlabeled dataset. 
These approaches assume known key states and require labeled in-domain finetuning data.
To the best of our knowledge, \gls{nils} is the only method that accurately labels real-world long-horizon robotic data without any model fine-tuning. 



==> Play_Labeling_Cam_Ready_arXiv/chapters/results_policy_plot.tex <==
\definecolor{ggreen_dark}{HTML}{008744}
\definecolor{ggreen_bright}{HTML}{4cab7c}

\definecolor{rred}{HTML}{C0504D}
\definecolor{ggreen}{HTML}{9BBB59}
\definecolor{ppurple}{HTML}{9F4C7C}

\centering
\begin{tikzpicture}
\begin{axis}[
ybar,
bar width=15pt,
width=0.45\columnwidth,
height=0.25\columnwidth,
symbolic x coords={Success, Correct Grounding},
nodes near coords,
nodes near coords align={vertical},
nodes near coords style={font=\tiny},
ymin=0,ymax=1.5,
ylabel={Success Rate},
xtick=data,
enlarge x limits=0.5,
x tick style={draw=none},
legend style={at={(0.5,-0.5)},font={\scriptsize},anchor=north,legend columns=-1},
ylabel near ticks,
ticklabel style = {font=\footnotesize},
extra y ticks = 4.5,
]
\addplot[color=ggreen_dark,fill=ggreen_dark] coordinates {(Success,0.47)(Correct Grounding,0.89)};
\addplot[color=ggreen_bright,fill=ggreen_bright] coordinates {(Success,0.278)(Correct Grounding,0.58)};
\addplot[color=rred,fill=rred] coordinates {(Success,0.58)(Correct Grounding,0.89)};
\legend{NILS,NILS Noisy,Human}
\end{axis}
\end{tikzpicture}




==> Play_Labeling_Cam_Ready_arXiv/chapters/rudi_method.tex <==
\section{Method}
\begin{figure}[t]
    \centering
   \includegraphics[width=\linewidth]{images/introduction/lupus_example.pdf}
   \vspace{-0.5cm}
    \caption{Overview of the proposed NILS framework for labeling long-horizon robot play sequences in a zero-shot manner using an ensemble of pretrained expert models.
    NILS consists of three Stages: First, all relevant objects in the video are detected. 
    In the second step, object-centric changes are detected and collected. 
    In Stage 3 the object change information is used to detect keystates and an LLM is prompted to generate a language label for the task.
    }
    \label{fig: lupus overview}
\end{figure}
\gls{nils} consists of three stages: \textit{Stage 1} (Identifying Objects in the Scene), \textit{Stage 2} (Object-Centric Scene Annotation), and \textit{Stage 3} (Keystate Detection and Label Generation).
\autoref{fig: lupus overview} depicts a comprehensive method overview. 
The subsequent sections elaborate on each stage.
\gls{nils} uses different frozen pretrained models across each state, which enable \textbf{modular replacement}.
A detailed list of the models used in \gls{nils}, including explanations and usage, is provided in \autoref{sec:add-lupus-details}.

\subsection{Stage 1: Identifying Objects in the Scene}
\label{sec:task_retrieval}

\looseness-1
In Stage 1, \gls{nils} deploys a set of VLMs to detect all objects and their relevant properties across multiple video frames.
This ensures comprehensive object detection even with occlusion.
\gls{nils} prompts the model to output concise and unique names for all objects in each frame. 
However, this approach results in inconsistent naming across frames for the same object.
To resolve this, \gls{nils} leverages \textit{temporal consensus}, \textit{co-occurrence}, and \textit{object detection alignment}.
It uses GroundingDINO~\cite{liu2023grounding} for bounding box generation and computes Intersection over Union (IOU) for co-occurrence.
\gls{nils} combines the detector confidence with a  SigLIP alignment score based on cropped image regions of the object.
Finally, an LLM assigns the properties \texttt{movable}, \texttt{is\_container}, \texttt{states}, and \texttt{interactable} to each object to help filter invalid robot-object interactions in later Stages.



\subsection{Stage 2: Object-Centric Scene Annotations}
Next, \gls{nils} generates object-centric scene annotations that allow to reason about robot-object interactions. 
For each object detected in Stage 1, \gls{nils} computes bounding boxes, segmentation masks, movement, relations, and state throughout the video.
The extracted information is used in Stage 3 to segment and annotate the demonstrations.
First, \gls{nils} identifies the object bounding boxes and segmentation masks to track various object changes.

\textbf{Object Annotations and Segmentations.}
\gls{nils} computes bounding boxes and segmentation masks for the robot manipulator and all objects from Stage 1 using an ensemble of open-vocabulary detection and segmentation models.
To address the detector confidence misalignment and class struggles, \gls{nils} ensembles the models by extracting bounding boxes for objects from Stage 1 (\autoref{sec:task_retrieval}).
Next, it computes the agreement between the detector and dense predictor inside each bounding box together with a temporal consensus approach.
A two-stage filtering process identifies the most representative bounding box to improve the detection robustness~\cite{dbscan}.
To address temporal misalignments and missing detections, \gls{nils} utilizes a mask-tracking model \cite{cheng2023tracking} to capture temporal correlations between objects.
Detailed explanations are provided in \autoref{sec:add-lupus-details}.

NILS monitors four main signals: (1) object relations and movement using segmentation masks, bounding boxes, and depth maps, (2) object state changes over time, (3) gripper position relative to objects, and (4) gripper closing and opening actions. These signals are used to generate templated language descriptions and identify key states throughout the video, which are then used to describe the overall task. 
Detailed descriptions on how we track individual signals are provided in \autoref{sec:ojbect-centric retrieval}.

\subsection{Stage 3: Keystate Detection and Label Generation}


Determining critical states that mark task boundaries is a key challenge in labeling long-horizon robot demonstrations.
\gls{nils} addresses this through a novel heuristic consensus method, using object-centric representations from Stage $2$ to detect individual manipulation tasks.
This method combines multiple heuristics to filter noise-induced false positives and identify reliable keystates.
\gls{nils} acquires object-centric keystates by having each heuristic monitor changes for objects to minimize the noise impact.
An object-centric keystate $o_i$ is considered valid if its score exceeds a threshold $\theta_o$
\begin{align}
S(o_i) = \sum_k \alpha_k * \text{S}_k({o}_i) ,
\end{align}
where $k$ is the heuristic index, $\alpha_k$ is the heuristic weight, and $S{k}(o_i)$ is the confidence of the current heuristic.
\gls{nils} uses equal weights for all heuristics.
The keystate score $S_k(o_i)$ controls the \textbf{quality} of generated keystates and language annotations (\autoref{fig:threshold-accuracy-relation}), providing an advantage over VLM captioning \cite{ren2023robots}.
\gls{nils} then aggregates nearby keystates and selects the highest-scoring one to minimize noise.

\textbf{Action Retrieval and Grounding}
After identifying keystates, \gls{nils} generates natural language descriptions of performed tasks.
It constructs templated language prompts based on the object-centric scene annotations in between detected keystates.
This information is used to query a LLM. 
The prompt focuses on a single object to help the LLM to concentrate on task-relevant information only. 
The LLM reasons about detected object movements and relation changes to determine possible robot actions.
\gls{nils} detected low-level keystates, and templated language observations can thus be aggregated. 
Combining multiple low-level language observations in a single prompt allows the LLM to reason about higher-level tasks, allowing control over the task \textbf{granularity}. 
We provide detailed explanations and examples in \autoref{sec:granulaity ablations}.
A list of example prompts is given in \autoref{sec:app_prompts}.


\subsection{Object-Centric Information Retrieval of Stage 2}
\label{sec:ojbect-centric retrieval}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.144\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/evaluation/env_vis/kitchen_play_1.png}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.192\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/evaluation/env_vis/bridge_1.png}
    \end{subfigure}%
    \hfill
    \hfill
    \begin{subfigure}[b]{0.192\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/evaluation/env_vis/bridge_4.png}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.192\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/evaluation/simpler/simpler_eval.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.192\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/evaluation/env_vis/fractal.png}
    \end{subfigure}%
    \caption{Overview of the environments used in our experiments. 
    From left to right: Toy kitchen setup, two scenes from the BridgeV2 dataset \cite{walke2024bridgedata}, one example task from the Simpler Eval \cite{li24simpler} and one scene from Fractal \cite{brohan2022rt}.}
    \label{fig:env_vis}
\end{figure}


We provide further details on the object-centric information retrieval in Stage 2. 
Using bounding boxes and the segmentation masks, \gls{nils} monitors various signals for labeling. 
\gls{nils} tracks the following signals to generate templated language with timestamps:



\textbf{Object Relations and Object Movement.}
\gls{nils} tracks object movement and relations using segmentation masks and bounding boxes.
It detects movement through bounding box displacement and flow-based detection \cite{xu2022gmflow} for small movements.
\gls{nils} constructs an object-relation graph with nodes representing objects and edges denoting spatial relations \cite{liu_reflect_2023}.
To capture depth-dependent relations (e.g., \texttt{inside, behind}), objects are projected onto a point cloud using a zero-shot depth map~\cite{yang2024depth}.
\gls{nils} generates templated language describing movement and spatial relations, e.g., \texttt{"[] moved to the left of []"}.
\gls{nils} generates \textbf{diverse} and informative labels based on these grounded scene observations, outperforming simple language-based paraphrasing methods.



\textbf{Object State Prediction.}
\gls{nils} predicts object states over time, which is crucial for static objects like drawers.
It crops object images from each frame and compares state text embeddings with image embeddings to determine the current object state.
To handle occlusion during robot interactions, NILS omits predictions when relevant objects are partially obscured.
The system generates templated language like \texttt{"Drawer changed from open to closed."}.

\textbf{Gripper Position.}
The gripper position over time indicates robot-object interactions.
\gls{nils} computes gripper-object proximity using object and robot segmentation masks and predicted depth map.
To account for end-effector position inaccuracies, a per-object threshold is used to determine contact.
A keystate is generated if the gripper-object distance is below the threshold for three frames with templated: \texttt{"The gripper was close to ..."}.

\textbf{Gripper Closing.}
When available, \gls{nils} uses gripper close signals as potential keystates.
\gls{nils} identifies a keystate when a previously closed gripper opens.

\gls{nils} collects these object changes and templated language observations throughout the video.


==> Play_Labeling_Cam_Ready_arXiv/lupus_macros.tex <==
\usepackage{xparse}
\usepackage[normalem]{ulem}

\usepackage{amssymb}
\newcommand{\conv}{\mathbin{\ast}}
\NewDocumentCommand\TODO{m}{\textcolor{red}{#1}}
\NewDocumentCommand\CHECK{m}{\textcolor{orange}{#1}}
\NewDocumentCommand\MORITZ{m}{\textcolor{blue}{#1}}
\NewDocumentCommand\CUT{m}{{\textcolor{red}{\sout{#1}}}}

\NewDocumentCommand\NewIndexedVar{mmm}{
\expandafter\NewDocumentCommand\csname#1\endcsname{se{^_}}{#2\IfNoValueTF{##2}{}{^{##2}}\IfNoValueTF{##3}{\IfBooleanTF{##1}{}{_#3}}{_{##3}}}
}




\usepackage[acronym]{glossaries}
\newacronym{lfp}{LfP}{Learning from Play}
\newacronym{mtil}{MTIL}{Multi-Task Imitation Learning}
\newacronym{mlp}{MLP}{Multi-Layer Perceptron}
\newacronym{nils}{NILS}{Natural language Instruction Labeling for Scalability}
\newacronym{mtact}{MT-ACT}{Multi-Task Action Chunking Transformer}



